Too Trivial To Test? An Inverse View on Defect Prediction to Identify Methods with Low Fault Risk

Background. Test resources are usually limited and therefore it is often not possible to completely test an application before a release. To cope with the problem of scarce resources, development teams can apply defect prediction to identify fault-prone code regions. However, defect prediction tends to low precision in cross-project prediction scenarios. Aims. We take an inverse view on defect prediction and aim to identify methods that can be deferred when testing because they contain hardly any faults due to their code being "trivial". We expect that characteristics of such methods might be project-independent, so that our approach could improve cross-project predictions. Method. We compute code metrics and apply association rule mining to create rules for identifying methods with low fault risk. We conduct an empirical study to assess our approach with six Java open-source projects containing precise fault data at the method level. Results. Our results show that inverse defect prediction can identify approx. 32-44% of the methods of a project to have a low fault risk; on average, they are about six times less likely to contain a fault than other methods. In cross-project predictions with larger, more diversified training sets, identified methods are even eleven times less likely to contain a fault. Conclusions. Inverse defect prediction supports the efficient allocation of test resources by identifying methods that can be treated with less priority in testing activities and is well applicable in cross-project prediction scenarios.

==> figures/55_Figure_Test_Split_10fold.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.9\linewidth]{./figures/graphics/Test_Split_single10f.pdf}
	\caption{\rqNumFaultsInLfr, \rqNumSizeLfr: 10-fold cross-validation.
						\formatCaptionDetails{For each of the ten stratified samples,
						 the classifier is trained on nine samples and tested on the methods of the tenth sample.}}
	\label{Fig:TestSplit10Fold}
\end{figure}

==> figures/55_Figure_Test_Split_5of6.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.9\linewidth]{./figures/graphics/Test_Split_5of6.pdf}
	\caption{\rqNumCrossPrj: Cross-project validation. 
					  \formatCaptionDetails{For each of the projects (here: \textit{Time}),
					  we used all other projects to compute association rules and test against the methods of the current project.}
					}
	\label{Fig:TestSplit5of6}
\end{figure}

==> figures/61_Figure_Classifications.tex <==
\begin{figure}
	\centering
	\includegraphics[width=1.0\linewidth]{./figures/graphics/Defect_Prediction_Relation_small.pdf}
	\vspace{-0.2cm}
		\caption[Defect prediction and IDP have different classification classes.]{
					 Defect prediction and IDP have different classification classes.
					 \formatCaptionDetails{
						Ideally, LFR methods are a possibly large subset of non-faulty methods
						and are not contained in the set of faulty methods.
					}}
	\label{Fig:ClassificationSets}
	\vspace{-0.25cm}
\end{figure}
